A Closer Look at Two of the Most Luminous Quasars in the Universe

Ultra-luminous quasars ($M_{1450} \leq -29$) provide us with a rare view into the nature of the most massive and most rapidly accreting supermassive black holes (SMBHs). Following the discovery of two of these extreme sources, J0341${+}$1720 ($M_{1450}=-29.56$, $z=3.71$) and J2125${-}$1719 ($M_{1450}=-29.39$, $z=3.90$), in the Extremely Luminous Quasar Survey (ELQS) and its extension to the Pan-STARRS\,1 footprint (PS-ELQS), we herein present an analysis of their rest-frame UV to optical spectroscopy. Both quasars harbor very massive SMBHs with $M_{\rm{BH}}=6.73_{-0.83}^{+0.75}\times10^{9}\,M_{\odot}$ and $M_{\rm{BH}}=5.45_{-0.55}^{+0.60}\times10^{9}\,M_{\odot}$, respectively, showing evidence of accretion above the Eddington limit ($L_{\rm{bol}}/L_{\rm{Edd}}=2.74_{-0.27}^{+0.39}$ and $L_{\rm{bol}}/L_{\rm{Edd}}=3.01_{-0.30}^{+0.34}$). NOEMA 3 millimeter observations of J0341${+}$1720 reveal a highly star-forming ($\rm{SFR}\approx1500\,M_{\odot}\,\rm{yr}^{-1}$), ultra-luminous infrared galaxy ($L_{\rm{TIR}}\approx1.0\times10^{13}\,L_{\odot}$) host, which, based on an estimate of its dynamical mass, is only ${\sim}30$ times more massive than the SMBH it harbors at its center. As examples of luminous super-Eddington accretion, these two quasars provide support for theories, which explain the existence of billion solar mass SMBHs ${\sim}700$ million years after the Big Bang by moderate super-Eddington growth from standard SMBH seeds.

==> A closer look at two of the most luminous quasars in the Universe/line_table.tex <==
\begin{deluxetable*}{ccccccc}
\tabletypesize{\footnotesize} 
\tablecaption{Emission line properties of J0341+1720 and J2125-1719 \label{tab:line_measurements}}
\tablehead{\colhead{Line} &\colhead{$z_{\rm{line, peak}}$} &\colhead{$F_{\rm{line}}$} &\colhead{FWHM$_{\rm{line}}$} &\colhead{EW$_{\rm{line}}$} &\colhead{$\Delta v({z_{\rm{line}}}{-}z_{\rm{sys}})$} & \colhead{Components}  \\ 
\nocolhead{} &\nocolhead{} &\colhead{($10^{-17}\,\rm{erg}\,\rm{s}^{-1}\rm{cm}^2$)} &\colhead{$(\rm{km}\,\rm{s}^{-1})$} &\colhead{(\AA)} &\colhead{$(\rm{km}\,\rm{s}^{-1})$} &\nocolhead{}} 
\startdata 
\multicolumn{7}{c}{J0341+1720} \\ 
\tableline\ion{Si}{4} &${3.6638}_{-0.0018}^{+0.0021}$ & ${2459.97}_{-134.59}^{+132.59}$ & ${7588}_{-329}^{+311}$ & ${7.11}_{-0.41}^{+0.41}$ & ${-2813}_{-114}^{+135}$ & 1G\\ 
\ion{C}{4} &${3.6691}_{-0.0013}^{+0.0013}$ & ${4419.30}_{-155.00}^{+127.42}$ & ${8484}_{-310}^{+261}$ & ${15.00}_{-0.58}^{+0.49}$ & ${-2473}_{-85}^{+85}$ & 1G\\ 
\ion{Mg}{2} &${3.7024}_{-0.0016}^{+0.0017}$ & ${783.69}_{-52.05}^{+59.00}$ & ${3551}_{-316}^{+362}$ & ${6.01}_{-0.40}^{+0.46}$ & ${-342}_{-105}^{+108}$ & 1G\\ 
\ion{Mg}{2} (VW01) &${3.7014}_{-0.0017}^{+0.0016}$ & ${929.43}_{-69.88}^{+68.58}$ & ${3922}_{-371}^{+407}$ & ${7.23}_{-0.55}^{+0.55}$ & ${-411}_{-111}^{+103}$ & 1G\\ 
$\rm{H}\beta$ &${3.7035}_{-0.0006}^{+0.0006}$ & ${2274.75}_{-70.91}^{+69.02}$ & ${3983}_{-255}^{+215}$ & ${45.90}_{-1.65}^{+1.59}$ & ${-275}_{-36}^{+38}$ & 2G\\ 
CO(4-3) & $3.7078\pm0.0005$ & \dots & $460\pm69$ & \dots & $0\pm69$ & 1G \\ 
\tableline\multicolumn{7}{c}{J2125-1719} \\ 
\tableline\ion{Si}{4} &${3.8886}_{-0.0003}^{+0.0003}$ & ${1615.57}_{-18.85}^{+17.39}$ & ${4193}_{-76}^{+42}$ & ${6.28}_{-0.08}^{+0.07}$ & ${-765}_{-17}^{+17}$ & 1G\\ 
\ion{C}{4} &${3.8983}_{-0.0019}^{+0.0026}$ & ${3887.95}_{-110.13}^{+177.84}$ & ${3246}_{-140}^{+126}$ & ${17.58}_{-0.50}^{+0.82}$ & ${-169}_{-117}^{+156}$ & 2G\\ 
$\rm{H}\beta$ &${3.9032}_{-0.0007}^{+0.0008}$ & ${1176.19}_{-28.00}^{+25.84}$ & ${3653}_{-189}^{+197}$ & ${31.58}_{-0.85}^{+0.73}$ & ${131}_{-42}^{+47}$ & 2G\\ 
$\rm{O[III]}\ \lambda4960\,$\AA &${3.9010}_{-0.0005}^{+0.0005}$ & ${139.26}_{-12.48}^{+13.36}$ & ${843}_{-95}^{+98}$ & ${3.81}_{-0.34}^{+0.37}$ & ${-6}_{-29}^{+32}$ & 1G\\ 
$\rm{O[III]}\ \lambda5007\,$\AA &${3.9011}_{-0.0003}^{+0.0003}$ & ${347.49}_{-16.36}^{+17.59}$ & ${811}_{-54}^{+47}$ & ${9.58}_{-0.45}^{+0.49}$ & ${-0}_{-17}^{+17}$ & 1G\\ 
\enddata 
\tablecomments{All line measurements of J0341{+}1720 are from the fit with the \citet{Tsuzuki2006} iron template with the exception of \ion{Mg}{2} (VW01), which was fit using the \citet{Vestergaard2001} iron template.} 
\end{deluxetable*} 


==> A closer look at two of the most luminous quasars in the Universe/prop_table.tex <==
\begin{deluxetable}{ccc}
\tabletypesize{\footnotesize} 
\tablecaption{Quasar properties directly measured or derived from the spectral fits \label{tab:fitproperties}}
\tablehead{\colhead{Measured Property} &\colhead{J0341+1720} &\colhead{J2125-1719} } 
\startdata 
$M_{1450}/(\rm{mag})$ &${-29.562}_{+0.004}^{-0.004}$ & ${-29.386}_{+0.001}^{-0.001}$\\ 
$L_{\rm{3000}} /(10^{46}\,\rm{erg}\,\rm{s}^{-1})$ & ${44.96}_{-0.21}^{+0.22}$ & ${40.13}_{-0.10}^{+0.11}$\\ 
$L_{\rm{3000}, VW01} /(10^{46}\,\rm{erg}\,\rm{s}^{-1})$ & ${44.98}_{-0.21}^{+0.20}$ &  \dots\\ 
$L_{\rm{5100}} /(10^{46}\,\rm{erg}\,\rm{s}^{-1})$ & ${27.22}_{-0.25}^{+0.25}$ & ${25.26}_{-0.13}^{+0.14}$\\ 
Power law index $\alpha$ & ${-1.620}_{-0.008}^{+0.007}$ & ${-1.551}_{-0.004}^{+0.004}$\\ 
$F_{\rm{FeII}}/F_{\rm{MgII}}$ & ${2.78}_{-0.65}^{+0.79}$ & \dots\\ 
\tableline Derived property & J0341+1720 & J2125-1719 \\ 
\tableline $L_{\rm{bol}} /(10^{48}\,\rm{erg}\,\rm{s}^{-1})$ & ${2.32}_{-0.01}^{+0.01}$ & ${2.07}_{-0.01}^{+0.01}$\\ 
MgII BH mass (VW09)/($10^{9}\,\rm{M}_{\odot}$) & ${7.47}_{-1.35}^{+1.63}$ & \dots\\ 
$\lambda_{\rm{Edd, MgII}}$ (VW09) & ${2.47}_{+0.54}^{-0.44}$ & \dots\\ 
H$\beta$ BH mass (VO06) ($10^{9}\,\rm{M}_{\odot}$) & ${6.73}_{-0.83}^{+0.75}$ & ${5.45}_{-0.55}^{+0.60}$\\ 
$\lambda_{\rm{Edd, H}\beta}$  (VO06) & ${2.74}_{+0.39}^{-0.27}$ & ${3.01}_{+0.34}^{-0.30}$\\ 
\ion{C}{4} BH mass (VO06) ($10^{9}\,\rm{M}_{\odot}$) & ${33.80}_{-2.43}^{+2.11}$ & ${4.53}_{-0.38}^{+0.36}$\\ 
$\lambda_{\rm{Edd,CIV}}$  (VO06) & ${0.55}_{+0.04}^{-0.03}$ & ${3.63}_{+0.33}^{-0.27}$\\ 
\ion{C}{4} BH mass (Co17) ($10^{9}\,\rm{M}_{\odot}$) & ${14.20}_{-1.16}^{+1.22}$ & \dots\\ 
$\lambda_{\rm{Edd,CIV}}$  (Co17) & ${1.30}_{-0.10}^{+0.12}$ & \dots\\ 
\enddata 
\tablerefs{VW01 : Iron template of \citet{Vestergaard2001}; VW09 : BH mass estimator of \citet{Vestergaard2009}; VO06 : BH mass estimator of \citet{Vestergaard2006}; Co17 : BH mass estimator of \citet{Coatman2017}} 
\tablecomments{All properties of J0341{+}1720 are from the fit with the \citet{Tsuzuki2006} iron template with the exception of $L_{3000,\rm{VW01}}$, for which the \citet{Vestergaard2001} iron template was used.} 
\end{deluxetable} 

